Tailoring Graph Neural Network-based Flow-guided Localization to Individual Bloodstreams and Activities

Flow-guided localization using in-body nanodevices in the bloodstream is expected to be beneficial for early disease detection, continuous monitoring of biological conditions, and targeted treatment. The nanodevices face size and power constraints that produce erroneous raw data for localization purposes. On-body anchors receive this data, and use it to derive the locations of diagnostic events of interest. Different Machine Learning (ML) approaches have been recently proposed for this task, yet they are currently restricted to a reference bloodstream of a resting patient. As such, they are unable to deal with the physical diversity of patients' bloodstreams and cannot provide continuous monitoring due to changes in individual patient's activities. Toward addressing these issues for the current State-of-the-Art (SotA) flow-guided localization approach based on Graph Neural Networks (GNNs), we propose a pipeline for GNN adaptation based on individual physiological indicators including height, weight, and heart rate. Our results indicate that the proposed adaptions are beneficial in reconciling the individual differences between bloodstreams and activities.

==> plot_region0.tex <==
%Define the color series
    \definecolor{RYB1}{RGB}{50,97,250}
    \definecolor{RYB2}{RGB}{50,150,250}
    \pgfplotscreateplotcyclelist{colorbrewer-RYB1}{
    {RYB1!50!black,fill=RYB1},
    {RYB1!50!black,fill=RYB1}} %Do not add a comma after the last element of the list!
    \pgfplotscreateplotcyclelist{colorbrewer-RYB2}{
    {RYB2!50!black,fill=RYB2},
    {RYB2!50!black,fill=RYB2}}
    
    %Define the width of the boxes
    \def\boxwidth{0.75}%
    
    % REGION 0
    \begin{tikzpicture}
    \begin{axis}[
        width=7.5 cm,
        axis on top,
        ymin=0, ymax=1,
        xmin=0, xmax=27,
        ylabel={Region accuracy},
        axis y line*=right,
        boxplot/draw direction=y,
        cycle list name=colorbrewer-RYB1,
        xtick={1.5, 4.5, 7.5, 10.5, 13.5, 16.5, 19.5, 22.5, 25.5},
        xticklabels={Original, Heavy, Light, Small, Short, Big, Tall, Active, Inactive},
        x tick label style={scale=1, rotate=65,align=center},
        tick align=inside,
        xtick style={draw=none},
        bar width=5pt
    ]
    
    \addplot+[ybar,thick]  
            plot coordinates {(2, 0.343179844)};
            
    \addplot+[ybar,thick]  
            plot coordinates {(5, 0.217202433)};
            
    \addplot+[ybar,thick]  
            plot coordinates {(8, 0.28931364)};
    
    \addplot+[ybar,thick]  
            plot coordinates {(11, 0.284969592)};
    
    \addplot+[ybar,thick]  
            plot coordinates {(14, 0.305821025)};
    
    \addplot+[ybar,thick]  
            plot coordinates {(17, 0.198088619)};
    
    \addplot+[ybar,thick]  
            plot coordinates {(20, 0.28931364)};
            
    \addplot+[ybar,thick]  
            plot coordinates {(23, 0.120764553)};
            
    \addplot+[ybar,thick]  
            plot coordinates {(26, 0.06602954)};
    

    \end{axis}
    \begin{axis}[
        width=7.5 cm,
        axis on top,
        ymin=0, ymax=1.5,
        xmin=0, xmax=27,
        boxplot/draw direction=y,
        ylabel={Point accuracy [m]},
        cycle list name=colorbrewer-RYB2,
        xtick={1.5, 4.5},
        xtick style={draw=none},
        axis y line*=left,
        axis x line=none
    ]
    \addplot+[
        boxplot={
            draw position=1,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region0_original_ptacc.csv};
    
    \addplot+[
        %boxplot prepared={draw position=4,
        boxplot ={draw position=4,
            %lower whisker=0,
            %lower quartile=0.25,
            %median=0.5,
            %average=0.5,
            %upper quartile=0.75,
            %upper whisker=1,
            average, % <---- Where is the average?
            box extend=\boxwidth
        }
    ]
    table[ y index=0, row sep=newline ]{region0_heavy_ptacc.csv};
    
    \addplot+[
        boxplot={
            draw position=7,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region0_light_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=10,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region0_small_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=13,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region0_short_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=16,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region0_big_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=19,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region0_tall_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=22,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region0_active_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=25,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region0_inactive_ptacc.csv};
    
    \end{axis}
    \end{tikzpicture}
    

==> plot_region1.tex <==
%Define the color series
    \definecolor{RYB1}{RGB}{50,97,250}
    \definecolor{RYB2}{RGB}{50,150,250}
    \pgfplotscreateplotcyclelist{colorbrewer-RYB1}{
    {RYB1!50!black,fill=RYB1},
    {RYB1!50!black,fill=RYB1}} %Do not add a comma after the last element of the list!
    \pgfplotscreateplotcyclelist{colorbrewer-RYB2}{
    {RYB2!50!black,fill=RYB2},
    {RYB2!50!black,fill=RYB2}}
    
    %Define the width of the boxes
    \def\boxwidth{0.75}%
    % REGION 2
    \begin{tikzpicture}
    \begin{axis}[
        width=7.5 cm,
        axis on top,
        ymin=0, ymax=1,
        xmin=0, xmax=27,
        ylabel={Region accuracy},
        axis y line*=right,
        boxplot/draw direction=y,
        cycle list name=colorbrewer-RYB1,
        xtick={1.5, 4.5, 7.5, 10.5, 13.5, 16.5, 19.5, 22.5, 25.5},
        xticklabels={Original, Heavy, Light, Small, Short, Big, Tall, Active, Inactive},
        x tick label style={scale=1, rotate=65,align=center},
        tick align=inside,
        xtick style={draw=none},
        bar width=5pt
    ]
    
    \addplot+[ybar,thick]  
            plot coordinates {(2, 0.322274882)};
            
    \addplot+[ybar,thick]  
            plot coordinates {(5, 0.240758294)};
            
    \addplot+[ybar,thick]  
            plot coordinates {(8, 0.314691943)};
    
    \addplot+[ybar,thick]  
            plot coordinates {(11, 0.274881517)};
    
    \addplot+[ybar,thick]  
            plot coordinates {(14, 0.265402844)};
    
    \addplot+[ybar,thick]  
            plot coordinates {(17, 0.234123223)};
    
    \addplot+[ybar,thick]  
            plot coordinates {(20, 0.296682464)};
            
    \addplot+[ybar,thick]  
            plot coordinates {(23, 0.161137441)};
            
    \addplot+[ybar,thick]  
            plot coordinates {(26, 0.026540284)};
    

    \end{axis}
    \begin{axis}[
        width=7.5 cm,
        axis on top,
        ymin=0, ymax=1.5,
        xmin=0, xmax=27,
        boxplot/draw direction=y,
        ylabel={Point accuracy [m]},
        cycle list name=colorbrewer-RYB2,
        xtick={1.5, 4.5},
        xtick style={draw=none},
        axis y line*=left,
        axis x line=none
    ]
    %Group A
    \addplot+[
        boxplot={
            draw position=1,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region1_original_ptacc.csv};
    
    %Group B
    \addplot+[
        %boxplot prepared={draw position=4,
        boxplot ={draw position=4,
            %lower whisker=0,
            %lower quartile=0.25,
            %median=0.5,
            %average=0.5,
            %upper quartile=0.75,
            %upper whisker=1,
            average, % <---- Where is the average?
            box extend=\boxwidth
        }
    ]
    table[ y index=0, row sep=newline ]{region1_heavy_ptacc.csv};
    
    \addplot+[
        boxplot={
            draw position=7,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region1_light_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=10,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region1_small_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=13,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region1_short_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=16,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region1_big_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=19,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region1_tall_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=22,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region1_active_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=25,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region1_inactive_ptacc.csv};
    
    \end{axis}
    \end{tikzpicture}
    

==> plot_region2.tex <==
%Define the color series
    \definecolor{RYB1}{RGB}{50,97,250}
    \definecolor{RYB2}{RGB}{50,150,250}
    \pgfplotscreateplotcyclelist{colorbrewer-RYB1}{
    {RYB1!50!black,fill=RYB1},
    {RYB1!50!black,fill=RYB1}} %Do not add a comma after the last element of the list!
    \pgfplotscreateplotcyclelist{colorbrewer-RYB2}{
    {RYB2!50!black,fill=RYB2},
    {RYB2!50!black,fill=RYB2}}
    
    %Define the width of the boxes
    \def\boxwidth{0.75}%
    
    % REGION 2
    \begin{tikzpicture}
    \begin{axis}[
        width=7.5 cm,
        axis on top,
        ymin=0, ymax=1,
        xmin=0, xmax=27,
        ylabel={Region accuracy},
        axis y line*=right,
        boxplot/draw direction=y,
        cycle list name=colorbrewer-RYB1,
        xtick={1.5, 4.5, 7.5, 10.5, 13.5, 16.5, 19.5, 22.5, 25.5},
        xticklabels={Original, Heavy, Light, Small, Short, Big, Tall, Active, Inactive},
        x tick label style={scale=1, rotate=65,align=center},
        tick align=inside,
        xtick style={draw=none},
        bar width=5pt
    ]
    
    \addplot+[ybar,thick]  
            plot coordinates {(2, 0.660826033)};
            
    \addplot+[ybar,thick]  
            plot coordinates {(5, 0.266583229)};
            
    \addplot+[ybar,thick]  
            plot coordinates {(8, 0.2077597)};
    
    \addplot+[ybar,thick]  
            plot coordinates {(11, 0.13767209)};
    
    \addplot+[ybar,thick]  
            plot coordinates {(14, 0.315394243)};
    
    \addplot+[ybar,thick]  
            plot coordinates {(17, 0.215269086)};
    
    \addplot+[ybar,thick]  
            plot coordinates {(20, 0.441802253)};
            
    \addplot+[ybar,thick]  
            plot coordinates {(23, 0.289111389)};
            
    \addplot+[ybar,thick]  
            plot coordinates {(26, 0.090112641)};
    

    \end{axis}
    \begin{axis}[
        width=7.5 cm,
        axis on top,
        ymin=0, ymax=1.5,
        xmin=0, xmax=27,
        boxplot/draw direction=y,
        ylabel={Point accuracy [m]},
        cycle list name=colorbrewer-RYB2,
        xtick={1.5, 4.5},
        xtick style={draw=none},
        axis y line*=left,
        axis x line=none
    ]
    %Group A
    \addplot+[
        boxplot={
            draw position=1,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region2_original_ptacc.csv};
    
    %Group B
    \addplot+[
        %boxplot prepared={draw position=4,
        boxplot ={draw position=4,
            %lower whisker=0,
            %lower quartile=0.25,
            %median=0.5,
            %average=0.5,
            %upper quartile=0.75,
            %upper whisker=1,
            average, % <---- Where is the average?
            box extend=\boxwidth
        }
    ]
    table[ y index=0, row sep=newline ]{region2_heavy_ptacc.csv};
    
    \addplot+[
        boxplot={
            draw position=7,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region2_light_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=10,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region2_small_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=13,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region2_short_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=16,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region2_big_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=19,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region2_tall_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=22,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region2_active_ptacc.csv};

    \addplot+[
        boxplot={
            draw position=25,
            average, % <---- Where is the average?
            box extend=\boxwidth
        },
    ]
    table[ y index=0, row sep=newline ]{region2_inactive_ptacc.csv};
    
    \end{axis}
    \end{tikzpicture}
    
